The geometry of random walk isomorphism theorems

The classical random walk isomorphism theorems relate the local times of a continuous-time random walk to the square of a Gaussian free field. A Gaussian free field is a spin system that takes values in Euclidean space, and this article generalises the classical isomorphism theorems to spin systems taking values in hyperbolic and spherical geometries. The corresponding random walks are no longer Markovian: they are the vertex-reinforced and vertex-diminished jump processes. We also investigate supersymmetric versions of these formulas. Our proofs are based on exploiting the continuous symmetries of the corresponding spin systems. The classical isomorphism theorems use the translation symmetry of Euclidean space, while in hyperbolic and spherical geometries the relevant symmetries are Lorentz boosts and rotations, respectively. These very short proofs are new even in the Euclidean case. Isomorphism theorems are useful tools, and to illustrate this we present several applications. These include simple proofs of exponential decay for spin system correlations, exact formulas for the resolvents of the joint processes of random walks together with their local times, and a new derivation of the Sabot--Tarr\`es formula for the limiting local time of the vertex-reinforced jump process.

==> localmacros.tex <==
\newcommand{\commentrb}[1]{\begin{quote} \cop \textbf{Comment from RB:} #1 \end{quote}}
\newcommand{\tyler}[1]{\begin{quote} \cop \textbf{Comment from Tyler:} #1 \end{quote}}
\newcommand{\commentandrew}[1]{\begin{quote} \cop \textbf{Comment from Andrew:} #1 \end{quote}}
\newcommand{\tylerc}[1]{{\cob #1}}

\newcommand{\Hhoro}{\widetilde H}
\newcommand{\Fhoro}{\widetilde F}
\newcommand{\Omegahoro}{\widetilde \Omega}
\newcommand{\ERRW}{\mathrm{ERRW}}
\newcommand{\VRJP}{\mathrm{VRJP}}
\newcommand{\V}[1]{\boldsymbol{#1}}

\newcommand{\co}[1]{\left[#1\right )} %% Closed then open braces
\newcommand{\oc}[1]{\left(#1\right ]} %% Open then closed braces
\newcommand{\ob}[1]{\left(#1\right )} %% Open braces
\newcommand{\cb}[1]{\left[#1\right ]} %% Closed braces

\newcommand{\death}{\zeta}
\newcommand{\cemetery}{\dagger}
\newcommand{\sdet}{\mathrm{sdet}}
\newcommand{\ball}{\bbB}

